Improving memory banks for unsupervised learning with large mini-batch, consistency and hard negative mining

An important component of unsupervised learning by instance-based discrimination is a memory bank for storing a feature representation for each training sample in the dataset. In this paper, we introduce 3 improvements to the vanilla memory bank-based formulation which brings massive accuracy gains: (a) Large mini-batch: we pull multiple augmentations for each sample within the same batch and show that this leads to better models and enhanced memory bank updates. (b) Consistency: we enforce the logits obtained by different augmentations of the same sample to be close without trying to enforce discrimination with respect to negative samples as proposed by previous approaches. (c) Hard negative mining: since instance discrimination is not meaningful for samples that are too visually similar, we devise a novel nearest neighbour approach for improving the memory bank that gradually merges extremely similar data samples that were previously forced to be apart by the instance level classification loss. Overall, our approach greatly improves the vanilla memory-bank based instance discrimination and outperforms all existing methods for both seen and unseen testing categories with cosine similarity.

==> figures/overall.tex <==
\newlength{\stackWidth}
\setlength{\stackWidth}{2cm}

\newlength{\smallestHeight}
\setlength{\smallestHeight}{12pt}

\tikzset{block2/.style={shape=rectangle, draw, node distance=-1pt, minimum width=\stackWidth, line width=1pt, inner sep=0pt}}

\begin{tikzpicture}

\definecolor{pozsample}{RGB}{251,141,60}
\definecolor{pozsample2}{RGB}{230,85,13}

\definecolor{blue0}{RGB}{31,120,180}
\definecolor{blue1}{RGB}{49,130,189}
\definecolor{blue2}{RGB}{107,174,214}
\definecolor{blue3}{RGB}{158,202,225}

\definecolor{netcolor}{RGB}{158,154,200}

\node[inner sep=0pt] (t0) at (0,0)
    {\includegraphics[width=.15\textwidth]{figures/01.jpg}};
\node [left=0.0cm of t0] {$\mathbf{x}_i^{(0)}$};

\node[circle,draw=black, fill=black, inner sep=0pt,minimum size=5pt, below=0.5cm of t0] (dot0) {};
\node[circle,draw=black, fill=black, inner sep=0pt,minimum size=5pt, below=0.2cm of dot0] (dot1) {};
\node[circle,draw=black, fill=black, inner sep=0pt,minimum size=5pt, below=0.2cm of dot1] (dot2) {};

\node[inner sep=0pt, below=2cm of t0] (t1)
    {\includegraphics[width=.15\textwidth]{figures/02.jpg}};
\node [left=0.0cm of t1] {$\mathbf{x}_i^{(k-2)}$};
\node[inner sep=0pt, below=0.5cm of t1] (t2)
    {\includegraphics[width=.15\textwidth]{figures/03.jpg}};
\node [left=0.0cm of t2] {$\mathbf{x}_i^{(k-1)}$};

\draw[black,thick,dotted] ($(t0.north west)+(-1.3,0.6)$)  rectangle ($(t2.south east)+(0.3,-0.6)$);

\node [trapezium, trapezium angle=80, minimum width=25mm, draw, thick, rotate=270,fill=netcolor] at ($0.5*(t0.north west)+0.5*(t2.south west)+(5.5,0.0)$) (cnn) {\rotatebox{90}{\textbf{CNN}}};

\draw [-latex] (t0.east) -- (cnn.south);
\draw [-latex] (t1.east) -- (cnn.south);
\draw [-latex] (t2.east) -- (cnn.south);

%\node[draw,thick,minimum width=2cm,minimum height=2cm]{};
% \path let \p{A}=(cnn.south west), \p{B}=(cnn.south east) in node[draw,thick,minimum width=0.5cm,minimum height=(\x{A}-\x{B})]{};
\node[draw,thick,minimum width=0.5cm,minimum height=2cm, right=1cm of cnn.north,fill=netcolor] (linear) {\rotatebox{90}{Linear}};

\node[draw,thick,minimum width=0.5cm,minimum height=2cm, right=1cm of linear.east,fill=netcolor] (l2) {\rotatebox{90}{$\ell_2 norm$}};

\draw [-latex] (cnn.north) -- (linear.west);
\draw [-latex] (linear.east) -- (l2.west);

\node[circle,minimum width=0.7cm,right=1cm of l2,fill=blue2] (sphere1) {}; %shading=ball
\node[thick,draw=black,circle,minimum width=0.7cm,right=1.7cm of sphere1] (sphere1-prod) {\large$\times$}; %shading=ball
\node [right=0.0cm of sphere1] (sphere1-text) {$\mathbf{f}_i^{(k-2)}$};
\node[circle,minimum width=0.7cm,above=1.5cm of sphere1,fill=blue1] (sphere2) {};
\node[thick,draw=black,circle,minimum width=0.7cm,right=1.7cm of sphere2] (sphere2-prod) {\large$\times$}; %shading=ball
\node [right=0.0cm of sphere2] (sphere2-text) {$\mathbf{f}_i^{(0)}$};
\node[circle,minimum width=0.7cm,below=1cm of sphere1,fill=blue3] (sphere3) {};
\node[thick,draw=black,circle,minimum width=0.7cm,right=1.7cm of sphere3] (sphere3-prod) {\large$\times$}; %shading=ball
\node [right=0.0cm of sphere3] (sphere3-text) {$\mathbf{f}_i^{(k-1)}$};

\draw [-latex,dashed] (sphere1-text.east) -- (sphere1-prod.west);
\draw [-latex,dashed] (sphere2-text.east) -- (sphere2-prod.west);
\draw [-latex,dashed] (sphere3-text.east) -- (sphere3-prod.west);

\draw[blue1,thick,dotted] ($(sphere2.north west)+(-0.2,0.2)$)  rectangle ($(sphere3.south east)+(0.2,-0.2)$);

\node[circle,draw=black,inner sep=0pt,minimum size=20pt, above=1.2cm of sphere2] (sum) {$\sum$};

\node[circle,draw=black, fill=black, inner sep=0pt,minimum size=5pt, below=0.3cm of sphere2] (dot0-1) {};
\node[circle,draw=black, fill=black, inner sep=0pt,minimum size=5pt, below=0.2cm of dot0-1] (dot1-1) {};
\node[circle,draw=black, fill=black, inner sep=0pt,minimum size=5pt, below=0.2cm of dot1-1] (dot2-2) {};

\draw [-latex] (linear.east) -- (l2.west);

\draw [-latex] (l2.east) -- (sphere1.west);
\draw [-latex] (l2.east) -- (sphere2.west);
\draw [-latex] (l2.east) -- (sphere3.west);

\draw [latex-latex,draw=pozsample2] (sphere1-prod) to [out=45,in=310] node [below, sloped] (TextNode1) {\small KL} (sphere2-prod);
\draw [latex-latex,draw=pozsample2] (sphere1-prod) to [out=315,in=50] node [above, sloped] (TextNode2) {\small KL} (sphere3-prod);
\draw [latex-latex,draw=pozsample2] (sphere3-prod) to [out=120,in=240] node [above, sloped,xshift=0.75cm] (TextNode1) {\small KL} (sphere2-prod);

\begin{scope}[every node/.style={block2}]
    \node[minimum height=2\smallestHeight,right=4cm of sphere1,align=center] (m-m) {\textbf{Memory}\\ \textbf{bank}};
    \node[minimum height=\smallestHeight,below=of m-m] (mb1) {$\mathbf{\hat{f}_{n-2}}$};
    \node[minimum height=\smallestHeight,below=of mb1] (mb2) {$\mathbf{\hat{f}_{n-2}}$};
    \node[minimum height=\smallestHeight,below=of mb2] (mb3) {$\mathbf{\hat{f}_{n-1}}$};
    
    \node[minimum height=\smallestHeight,above=of m-m] (m1) {$\cdots$};
    \node[minimum height=\smallestHeight,above=of m1,fill=blue0] (m2) {$\mathbf{\hat{f}_i}$};
    \node[minimum height=\smallestHeight,above=of m2] (m3) {$\cdots$};
    \node[minimum height=\smallestHeight,above=of m3] (m4) {$\mathbf{\hat{f}_0}$};
\end{scope}

\draw [decorate,decoration={brace,amplitude=10pt,mirror},xshift=4pt,yshift=0pt]($(m4.north west)+(0.0,0)$) -- ($(mb3.south west)+(0.0,0)$) node [black,midway,xshift=-0.6cm] (decoration-mem) {};

\draw [-latex,dashed] (decoration-mem.east) -- (sphere3-prod.east);
\draw [-latex,dashed] (decoration-mem.east) -- (sphere2-prod.east);
\draw [-latex,dashed] (decoration-mem.east) -- (sphere1-prod.east);

% \draw[decoration = {zigzag,segment length = 3mm, amplitude = 1mm},decorate] ($(m3.north)+(0.0,0.75)$)--($(m3.north)+(0.0,3.5)$);
\draw [-latex, dotted] ($(sphere2.north)+(0.0,0.2)$) -- (sum.south);
\draw [-latex, dotted] (sum.east) -- node[above,xshift=-1.25cm] {} ($(sum.east)+(7.0,0.0)$) -- ($(m2.east)+(0.95,0.0)$) -- (m2.east);
%$\times(1-m)$

% \node [] at ($(m3.north)+(-1.0,3.2)$) (t0) {\Large$\mathbf{t}$};
% \node [] at ($(m3.north)+(1.0,3.2)$) (t1) {\Large$\mathbf{t+1}$};
% add a, b, c
\end{tikzpicture}
